Non-thermal CMSSM with a 125 GeV Higgs

We study the phenomenology of the CMSSM/mSUGRA with non-thermal neutralino dark matter. Besides the standard parameters of the CMSSM we include the reheating temperature as an extra parameter. Imposing radiative electroweak symmetry breaking with a Higgs mass around 125 GeV and no dark matter overproduction, we contrast the scenario with different experimental bounds from colliders (LEP, LHC), cosmic microwave background (Planck), direct (LUX, XENON100, CDMS, IceCube) and indirect (Fermi) dark matter searches. The allowed parameter space is characterised by a Higgsino-like LSP with a mass around 300 GeV. The observed dark matter abundance can be saturated for reheating temperatures around 2 GeV while larger temperatures require extra non-neutralino dark matter candidates and extend the allowed parameter space. Sfermion and gluino masses are in the few TeV region. These scenarios can be achieved in string models of sequestered supersymmetry breaking which avoid cosmological moduli problems and are compatible with gauge coupling unification. Astrophysics and particle physics experiments will fully investigate this non-thermal scenario in the near future.

==> biblio <==
@article{Aparicio:2014wxa,
      author         = "Aparicio, Luis and Cicoli, Michele and Krippendorf, Sven
                        and Maharana, Anshuman and Muia, Francesco and others",
      title          = "{Sequestered de Sitter String Scenarios: Soft-terms}",
      journal        = "JHEP",
      volume         = "1411",
      pages          = "071",
      doi            = "10.1007/JHEP11(2014)071",
      year           = "2014",
      eprint         = "1409.1931",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1409.1931;%%",
}

@article{Acharya:2008bk,
      author         = "Acharya, Bobby Samir and Kumar, Piyush and Bobkov,
                        Konstantin and Kane, Gordon and Shao, Jing and others",
      title          = "{Non-thermal Dark Matter and the Moduli Problem in String
                        Frameworks}",
      journal        = "JHEP",
      volume         = "0806",
      pages          = "064",
      doi            = "10.1088/1126-6708/2008/06/064",
      year           = "2008",
      eprint         = "0804.0863",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCB-PTH-08-06, MCTP-08-10",
      SLACcitation   = "%%CITATION = ARXIV:0804.0863;%%",
}

@article{Allahverdi:2014ppa,
      author         = "Allahverdi, Rouzbeh and Cicoli, Michele and Dutta,
                        Bhaskar and Sinha, Kuver",
      title          = "{Correlation between Dark Matter and Dark Radiation in
                        String Compactifications}",
      journal        = "JCAP",
      volume         = "1410",
      pages          = "002",
      doi            = "10.1088/1475-7516/2014/10/002",
      year           = "2014",
      eprint         = "1401.4364",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1401.4364;%%",
}

@article{Dutta:2009uf,
      author         = "Dutta, Bhaskar and Leblond, Louis and Sinha, Kuver",
      title          = "{Mirage in the Sky: Non-thermal Dark Matter, Gravitino
                        Problem, and Cosmic Ray Anomalies}",
      journal        = "Phys.Rev.",
      volume         = "D80",
      pages          = "035014",
      doi            = "10.1103/PhysRevD.80.035014",
      year           = "2009",
      eprint         = "0904.3773",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MIFP-09-19, NSF-KITP-09-52",
      SLACcitation   = "%%CITATION = ARXIV:0904.3773;%%",
}

@article{Allahverdi:2013noa,
      author         = "Allahverdi, Rouzbeh and Cicoli, Michele and Dutta,
                        Bhaskar and Sinha, Kuver",
      title          = "{Nonthermal dark matter in string compactifications}",
      journal        = "Phys.Rev.",
      number         = "9",
      volume         = "D88",
      pages          = "095015",
      doi            = "10.1103/PhysRevD.88.095015",
      year           = "2013",
      eprint         = "1307.5086",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1307.5086;%%",
}

@article{Lowen:2008fm,
      author         = "Lowen, Valeri and Nilles, Hans Peter",
      title          = "{Mirage Pattern from the Heterotic String}",
      journal        = "Phys.Rev.",
      volume         = "D77",
      pages          = "106007",
      doi            = "10.1103/PhysRevD.77.106007",
      year           = "2008",
      eprint         = "0802.1137",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0802.1137;%%",
}
@article{Craig:2013cxa,
      author         = "Craig, Nathaniel",
      title          = "{The State of Supersymmetry after Run I of the LHC}",
      year           = "2013",
      eprint         = "1309.0528",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1309.0528;%%",
}
@article{Ibanez:2007tu,
      author         = "Ibanez, L.E. and Uranga, A.M.",
      title          = "{Instanton induced open string superpotentials and branes
                        at singularities}",
      journal        = "JHEP",
      volume         = "0802",
      pages          = "103",
      doi            = "10.1088/1126-6708/2008/02/103",
      year           = "2008",
      eprint         = "0711.1316",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "IFT-UAM-CSIC-07-57, CERN-PH-TH-2007-215",
      SLACcitation   = "%%CITATION = ARXIV:0711.1316;%%",
}

@article{Brust:2011tb,
      author         = "Brust, Christopher and Katz, Andrey and Lawrence, Scott
                        and Sundrum, Raman",
      title          = "{SUSY, the Third Generation and the LHC}",
      journal        = "JHEP",
      volume         = "1203",
      pages          = "103",
      doi            = "10.1007/JHEP03(2012)103",
      year           = "2012",
      eprint         = "1110.6670",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UMD-PP-011-017",
      SLACcitation   = "%%CITATION = ARXIV:1110.6670;%%",
}
@article{Krippendorf:2013dqa,
      author         = "Krippendorf, Sven and Nilles, Hans Peter and Ratz,
                        Michael and Winkler, Martin Wolfgang",
      title          = "{Hidden SUSY from precision gauge unification}",
      journal        = "Phys.Rev.",
      volume         = "D88",
      pages          = "035022",
      doi            = "10.1103/PhysRevD.88.035022",
      year           = "2013",
      eprint         = "1306.0574",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-13-099, TUM-HEP-892-13, FLAVOR-EU-43",
      SLACcitation   = "%%CITATION = ARXIV:1306.0574;%%",
}
@article{Krippendorf:2012ir,
      author         = "Krippendorf, Sven and Nilles, Hans Peter and Ratz,
                        Michael and Winkler, Martin Wolfgang",
      title          = "{The heterotic string yields natural supersymmetry}",
      journal        = "Phys.Lett.",
      volume         = "B712",
      pages          = "87-92",
      doi            = "10.1016/j.physletb.2012.04.043",
      year           = "2012",
      eprint         = "1201.4857",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1201.4857;%%",
}
@article{Badziak:2012yg,
      author         = "Badziak, Marcin and Krippendorf, Sven and Nilles, Hans
                        Peter and Winkler, Martin Wolfgang",
      title          = "{The heterotic MiniLandscape and the 126 GeV Higgs
                        boson}",
      journal        = "JHEP",
      volume         = "1303",
      pages          = "094",
      doi            = "10.1007/JHEP03(2013)094",
      year           = "2013",
      eprint         = "1212.0854",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-12-230",
      SLACcitation   = "%%CITATION = ARXIV:1212.0854;%%",
}
@article{Ross:2012nr,
      author         = "Ross, Graham G. and Schmidt-Hoberg, Kai and Staub,
                        Florian",
      title          = "{The Generalised NMSSM at One Loop: Fine Tuning and
                        Phenomenology}",
      journal        = "JHEP",
      volume         = "1208",
      pages          = "074",
      doi            = "10.1007/JHEP08(2012)074",
      year           = "2012",
      eprint         = "1205.1509",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "OUTP-12-06P, BONN-TH-2012-04",
      SLACcitation   = "%%CITATION = ARXIV:1205.1509;%%",
}
@article{Papucci:2011wy,
      author         = "Papucci, Michele and Ruderman, Joshua T. and Weiler,
                        Andreas",
      title          = "{Natural SUSY Endures}",
      journal        = "JHEP",
      volume         = "1209",
      pages          = "035",
      doi            = "10.1007/JHEP09(2012)035",
      year           = "2012",
      eprint         = "1110.6926",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-11-193, CERN-PH-TH-265",
      SLACcitation   = "%%CITATION = ARXIV:1110.6926;%%",
}
@article{Allanach:2012vj,
      author         = "Allanach, B.C. and Gripaios, Ben",
      title          = "{Hide and Seek With Natural Supersymmetry at the LHC}",
      journal        = "JHEP",
      volume         = "1205",
      pages          = "062",
      doi            = "10.1007/JHEP05(2012)062",
      year           = "2012",
      eprint         = "1202.6616",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1202.6616;%%",
}

@article{Kitano:2005ew,
      author         = "Kitano, Ryuichiro and Nomura, Yasunori",
      title          = "{Dark matter before the LHC in a natural supersymmetric
                        standard model}",
      journal        = "Phys.Lett.",
      volume         = "B632",
      pages          = "162-166",
      doi            = "10.1016/j.physletb.2005.10.069",
      year           = "2006",
      eprint         = "hep-ph/0509221",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SLAC-PUB-11487, UCB-PTH-05-29, LBNL-58876",
      SLACcitation   = "%%CITATION = HEP-PH/0509221;%%",
}

@article{Baer:2012uy,
      author         = "Baer, Howard and Barger, Vernon and Huang, Peisi and
                        Tata, Xerxes",
      title          = "{Natural Supersymmetry: LHC, dark matter and ILC
                        searches}",
      journal        = "JHEP",
      volume         = "1205",
      pages          = "109",
      doi            = "10.1007/JHEP05(2012)109",
      year           = "2012",
      eprint         = "1203.5539",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UH-511-1190-12",
      SLACcitation   = "%%CITATION = ARXIV:1203.5539;%%",
}

@article{Nilles:1997cm,
      author         = "Nilles, Hans Peter and Olechowski, M. and Yamaguchi,
                        Masahiro",
      title          = "{Supersymmetry breaking and soft terms in M theory}",
      journal        = "Phys.Lett.",
      volume         = "B415",
      pages          = "24-30",
      doi            = "10.1016/S0370-2693(97)01212-4",
      year           = "1997",
      eprint         = "hep-th/9707143",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "TUM-HEP-282-97, SFB-375-201",
      SLACcitation   = "%%CITATION = HEP-TH/9707143;%%",
}


@article{Acharya:2008zi,
      author         = "Acharya, Bobby Samir and Bobkov, Konstantin and Kane,
                        Gordon L. and Shao, Jing and Kumar, Piyush",
      title          = "{The G(2)-MSSM: An M Theory motivated model of Particle
                        Physics}",
      journal        = "Phys.Rev.",
      volume         = "D78",
      pages          = "065038",
      doi            = "10.1103/PhysRevD.78.065038",
      year           = "2008",
      eprint         = "0801.0478",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MCTP-07-43, UCB-PTH-08-01",
      SLACcitation   = "%%CITATION = ARXIV:0801.0478;%%",
}

@article{Cicoli:2013rwa,
      author         = "Cicoli, Michele and de Alwis, Senarath and Westphal,
                        Alexander",
      title          = "{Heterotic Moduli Stabilisation}",
      journal        = "JHEP",
      volume         = "1310",
      pages          = "199",
      doi            = "10.1007/JHEP10(2013)199",
      year           = "2013",
      eprint         = "1304.1809",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DESY-13-066",
      SLACcitation   = "%%CITATION = ARXIV:1304.1809;%%",
}

@article{Evans:2012bf,
      author         = "Evans, Jared A. and Kats, Yevgeny",
      title          = "{LHC Coverage of RPV MSSM with Light Stops}",
      journal        = "JHEP",
      volume         = "1304",
      pages          = "028",
      doi            = "10.1007/JHEP04(2013)028",
      year           = "2013",
      eprint         = "1209.0764",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "RUNHETC-2012-18",
      SLACcitation   = "%%CITATION = ARXIV:1209.0764;%%",
}

@article{LeCompte:2011cn,
      author         = "LeCompte, Thomas J. and Martin, Stephen P.",
      title          = "{Large Hadron Collider reach for supersymmetric models
                        with compressed mass spectra}",
      journal        = "Phys.Rev.",
      volume         = "D84",
      pages          = "015004",
      doi            = "10.1103/PhysRevD.84.015004",
      year           = "2011",
      eprint         = "1105.4304",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ANL-HEP-PR-11-32, FERMILAB-PUB-11-903-T",
      SLACcitation   = "%%CITATION = ARXIV:1105.4304;%%",
}

@article{Conlon:2005ki,
      author         = "Conlon, Joseph P. and Quevedo, Fernando and Suruliz,
                        Kerim",
      title          = "{Large-volume flux compactifications: Moduli spectrum and
                        D3/D7 soft supersymmetry breaking}",
      journal        = "JHEP",
      volume         = "0508",
      pages          = "007",
      doi            = "10.1088/1126-6708/2005/08/007",
      year           = "2005",
      eprint         = "hep-th/0505076",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2005-48",
      SLACcitation   = "%%CITATION = HEP-TH/0505076;%%",
}
@article{Berg:2012aq,
      author         = "Berg, Marcus and Conlon, Joseph P. and Marsh, David and
                        Witkowski, Lukas T.",
      title          = "{Superpotential de-sequestering in string models}",
      journal        = "JHEP",
      volume         = "1302",
      pages          = "018",
      doi            = "10.1007/JHEP02(2013)018",
      year           = "2013",
      eprint         = "1207.1103",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1207.1103;%%",
}
@article{Conlon:2008wa,
      author         = "Conlon, Joseph P. and Maharana, Anshuman and Quevedo,
                        Fernando",
      title          = "{Towards Realistic String Vacua}",
      journal        = "JHEP",
      volume         = "0905",
      pages          = "109",
      doi            = "10.1088/1126-6708/2009/05/109",
      year           = "2009",
      eprint         = "0810.5660",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "OUTP-08-18P, DAMTP-2008-101, CERN-PH-TH-2008-214",
      SLACcitation   = "%%CITATION = ARXIV:0810.5660;%%",
}
@article{Ibanez:2014zsa,
      author         = "Ibanez, Luis E. and Valenzuela, Irene",
      title          = "{BICEP2, the Higgs Mass and the SUSY-breaking Scale}",
      year           = "2014",
      eprint         = "1403.6081",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-UAM-CSIC-14-026",
      SLACcitation   = "%%CITATION = ARXIV:1403.6081;%%",
}
@article{Grimm:2013bha,
      author         = "Grimm, Thomas W. and Keitel, Jan and Savelli, Raffaele
                        and Weissenbacher, Matthias",
      title          = "{From M-theory higher curvature terms to $\alpha'$
                        corrections in F-theory}",
      year           = "2013",
      eprint         = "1312.1376",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1312.1376;%%",
}
@article{Conlon:2009xf,
      author         = "Conlon, Joseph P.",
      title          = "{Gauge Threshold Corrections for Local String Models}",
      journal        = "JHEP",
      volume         = "0904",
      pages          = "059",
      doi            = "10.1088/1126-6708/2009/04/059",
      year           = "2009",
      eprint         = "0901.4350",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "OUTP-09-03P",
      SLACcitation   = "%%CITATION = ARXIV:0901.4350;%%",
}
@article{Burgess:2010sy,
      author         = "Burgess, C.P. and Maharana, Anshuman and Quevedo, F.",
      title          = "{Uber-naturalness: unexpectedly light scalars from
                        supersymmetric extra dimensions}",
      journal        = "JHEP",
      volume         = "1105",
      pages          = "010",
      doi            = "10.1007/JHEP05(2011)010",
      year           = "2011",
      eprint         = "1005.1199",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "IC-2010-013, DAMTP-2010-31",
      SLACcitation   = "%%CITATION = ARXIV:1005.1199;%%",
}
@article{Berg:2010ha,
      author         = "Berg, Marcus and Marsh, David and McAllister, Liam and
                        Pajer, Enrico",
      title          = "{Sequestering in String Compactifications}",
      journal        = "JHEP",
      volume         = "1106",
      pages          = "134",
      doi            = "10.1007/JHEP06(2011)134",
      year           = "2011",
      eprint         = "1012.1858",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1012.1858;%%",
}

@article{Conlon:2009kt,
      author         = "Conlon, Joseph P. and Palti, Eran",
      title          = "{Gauge Threshold Corrections for Local Orientifolds}",
      journal        = "JHEP",
      volume         = "0909",
      pages          = "019",
      doi            = "10.1088/1126-6708/2009/09/019",
      year           = "2009",
      eprint         = "0906.1920",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "OUTP-09-13P",
      SLACcitation   = "%%CITATION = ARXIV:0906.1920;%%",
}

@article{Choi:2005ge,
      author         = "Choi, Kiwoon and Falkowski, Adam and Nilles, Hans Peter
                        and Olechowski, Marek",
      title          = "{Soft supersymmetry breaking in KKLT flux
                        compactification}",
      journal        = "Nucl.Phys.",
      volume         = "B718",
      pages          = "113-133",
      doi            = "10.1016/j.nuclphysb.2005.04.032",
      year           = "2005",
      eprint         = "hep-th/0503216",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "IFT-05-05, KAIST-TH-2005-04, DESY-05-052",
      SLACcitation   = "%%CITATION = HEP-TH/0503216;%%",
}
@article{Acharya:2012tw,
      author         = "Acharya, Bobby Samir and Kane, Gordon and Kumar, Piyush",
      title          = "{Compactified String Theories -- Generic Predictions for
                        Particle Physics}",
      journal        = "Int.J.Mod.Phys.",
      volume         = "A27",
      pages          = "1230012",
      doi            = "10.1142/S0217751X12300128",
      year           = "2012",
      eprint         = "1204.2795",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1204.2795;%%",
}
@article{Kachru:2003aw,
      author         = "Kachru, Shamit and Kallosh, Renata and Linde, Andrei D.
                        and Trivedi, Sandip P.",
      title          = "{De Sitter vacua in string theory}",
      journal        = "Phys.Rev.",
      volume         = "D68",
      pages          = "046005",
      doi            = "10.1103/PhysRevD.68.046005",
      year           = "2003",
      eprint         = "hep-th/0301240",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "SLAC-PUB-9630, SU-ITP-03-01, TIFR-TH-03-03",
      SLACcitation   = "%%CITATION = HEP-TH/0301240;%%",
}
@article{Camara:2003ku,
      author         = "Camara, Pablo G. and Ibanez, L.E. and Uranga, A.M.",
      title          = "{Flux induced SUSY breaking soft terms}",
      journal        = "Nucl.Phys.",
      volume         = "B689",
      pages          = "195-242",
      doi            = "10.1016/j.nuclphysb.2004.04.013",
      year           = "2004",
      eprint         = "hep-th/0311241",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "IFT-UAM-CSIC-03-42",
      SLACcitation   = "%%CITATION = HEP-TH/0311241;%%",
}
@article{Conlon:2011jq,
      author         = "Conlon, Joseph P. and Witkowski, Lukas T.",
      title          = "{Scattering and Sequestering of Blow-Up Moduli in Local
                        String Models}",
      journal        = "JHEP",
      volume         = "1112",
      pages          = "028",
      doi            = "10.1007/JHEP12(2011)028",
      year           = "2011",
      eprint         = "1109.4153",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "OUTP-11-51P",
      SLACcitation   = "%%CITATION = ARXIV:1109.4153;%%",
}
@article{Conlon:2013isa,
      author         = "Conlon, Joseph P. and Marsh, M. C. David",
      title          = "{The Cosmophenomenology of Axionic Dark Radiation}",
      journal        = "JHEP",
      volume         = "1310",
      pages          = "214",
      doi            = "10.1007/JHEP10(2013)214",
      year           = "2013",
      eprint         = "1304.1804",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1304.1804;%%",
}
@article{Cicoli:2014sva,
      author         = "Cicoli, Michele and Dutta, Koushik and Maharana,
                        Anshuman",
      title          = "{N-flation with Hierarchically Light Axions in String
                        Compactifications}",
      year           = "2014",
      eprint         = "1401.2579",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "HRI-ST1402, SINP-TNP-2014-19",
      SLACcitation   = "%%CITATION = ARXIV:1401.2579;%%",
}
@article{Conlon:2008cj,
      author         = "Conlon, Joseph P. and Kallosh, Renata and Linde, Andrei
                        D. and Quevedo, Fernando",
      title          = "{Volume Modulus Inflation and the Gravitino Mass
                        Problem}",
      journal        = "JCAP",
      volume         = "0809",
      pages          = "011",
      doi            = "10.1088/1475-7516/2008/09/011",
      year           = "2008",
      eprint         = "0806.0809",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2007-36, CAV-HEP-08-07, YITP-08-42",
      SLACcitation   = "%%CITATION = ARXIV:0806.0809;%%",
}
@article{Kallosh:2004yh,
      author         = "Kallosh, Renata and Linde, Andrei D.",
      title          = "{Landscape, the scale of SUSY breaking, and inflation}",
      journal        = "JHEP",
      volume         = "0412",
      pages          = "004",
      doi            = "10.1088/1126-6708/2004/12/004",
      year           = "2004",
      eprint         = "hep-th/0411011",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = HEP-TH/0411011;%%",
}
@article{Aparicio:2008wh,
      author         = "Aparicio, L. and Cerdeno, D.G. and Ibanez, L.E.",
      title          = "{Modulus-dominated SUSY-breaking soft terms in F-theory
                        and their test at LHC}",
      journal        = "JHEP",
      volume         = "0807",
      pages          = "099",
      doi            = "10.1088/1126-6708/2008/07/099",
      year           = "2008",
      eprint         = "0805.2943",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-UAM-CSIC-08-27",
      SLACcitation   = "%%CITATION = ARXIV:0805.2943;%%",
}
@article{Conlon:2006tj,
      author         = "Conlon, Joseph P. and Cremades, Daniel and Quevedo,
                        Fernando",
      title          = "{Kahler potentials of chiral matter fields for Calabi-Yau
                        string compactifications}",
      journal        = "JHEP",
      volume         = "0701",
      pages          = "022",
      doi            = "10.1088/1126-6708/2007/01/022",
      year           = "2007",
      eprint         = "hep-th/0609180",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2006-79, NSF-KITP-06-81",
      SLACcitation   = "%%CITATION = HEP-TH/0609180;%%",
}
@article{Conlon:2013txa,
      author         = "Conlon, Joseph P. and Marsh, M. C. David",
      title          = "{Searching for a 0.1-1 keV Cosmic Axion Background}",
      journal        = "Phys.Rev.Lett.",
      volume         = "111",
      pages          = "151301",
      doi            = "10.1103/PhysRevLett.111.151301",
      year           = "2013",
      eprint         = "1305.3603",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1305.3603;%%",
}
@article{Hebecker:2013lha,
      author         = "Hebecker, Arthur and Knochel, Alexander K. and Weigand,
                        Timo",
      title          = "{The Higgs mass from a String-Theoretic Perspective}",
      journal        = "Nucl.Phys.",
      volume         = "B874",
      pages          = "1-35",
      doi            = "10.1016/j.nuclphysb.2013.05.004",
      year           = "2013",
      eprint         = "1304.2767",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1304.2767;%%",
}
@article{Lebedev:2005ge,
      author         = "Lebedev, Oleg and Nilles, Hans Peter and Ratz, Michael",
      title          = "{A Note on fine-tuning in mirage mediation}",
      pages          = "211-221",
      year           = "2005",
      eprint         = "hep-ph/0511320",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0511320;%%",
}
@article{Arvanitaki:2012ps,
      author         = "Arvanitaki, Asimina and Craig, Nathaniel and Dimopoulos,
                        Savas and Villadoro, Giovanni",
      title          = "{Mini-Split}",
      journal        = "JHEP",
      volume         = "1302",
      pages          = "126",
      doi            = "10.1007/JHEP02(2013)126",
      year           = "2013",
      eprint         = "1210.0555",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1210.0555;%%",
}


@article{Choi:2005hd,
      author         = "Choi, Kiwoon and Jeong, Kwang Sik and Kobayashi, Tatsuo
                        and Okumura, Ken-ichi",
      title          = "{Little SUSY hierarchy in mixed modulus-anomaly
                        mediation}",
      journal        = "Phys.Lett.",
      volume         = "B633",
      pages          = "355-361",
      doi            = "10.1016/j.physletb.2005.11.078",
      year           = "2006",
      eprint         = "hep-ph/0508029",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KAIST-TH-2005-12, KUNS-1982, KYUSHU-HET-85",
      SLACcitation   = "%%CITATION = HEP-PH/0508029;%%",
}

@article{Blumenhagen:2009gk,
      author         = "Blumenhagen, R. and Conlon, J.P. and Krippendorf, S. and
                        Moster, S. and Quevedo, F.",
      title          = "{SUSY Breaking in Local String/F-Theory Models}",
      journal        = "JHEP",
      volume         = "0909",
      pages          = "007",
      doi            = "10.1088/1126-6708/2009/09/007",
      year           = "2009",
      eprint         = "0906.3297",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "MPP-2009-76, OUTP-09-14P, DAMTP-2009-48,
                        CERN-PH-TH-2009-089",
      SLACcitation   = "%%CITATION = ARXIV:0906.3297;%%",
}

@article{Balasubramanian:2005zx,
      author         = "Balasubramanian, Vijay and Berglund, Per and Conlon,
                        Joseph P. and Quevedo, Fernando",
      title          = "{Systematics of moduli stabilisation in Calabi-Yau flux
                        compactifications}",
      journal        = "JHEP",
      volume         = "0503",
      pages          = "007",
      doi            = "10.1088/1126-6708/2005/03/007",
      year           = "2005",
      eprint         = "hep-th/0502058",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2005-10, UNH-05-01, UPR-1109-T",
      SLACcitation   = "%%CITATION = HEP-TH/0502058;%%",
}
@article{Bousso:2000xa,
      author         = "Bousso, Raphael and Polchinski, Joseph",
      title          = "{Quantization of four form fluxes and dynamical
                        neutralization of the cosmological constant}",
      journal        = "JHEP",
      volume         = "0006",
      pages          = "006",
      doi            = "10.1088/1126-6708/2000/06/006",
      year           = "2000",
      eprint         = "hep-th/0004134",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "SU-ITP-00-12, NSF-ITP-00-40",
      SLACcitation   = "%%CITATION = HEP-TH/0004134;%%",
}
@article{ArkaniHamed:2004fb,
      author         = "Arkani-Hamed, Nima and Dimopoulos, Savas",
      title          = "{Supersymmetric unification without low energy
                        supersymmetry and signatures for fine-tuning at the LHC}",
      journal        = "JHEP",
      volume         = "0506",
      pages          = "073",
      doi            = "10.1088/1126-6708/2005/06/073",
      year           = "2005",
      eprint         = "hep-th/0405159",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = HEP-TH/0405159;%%",
}

@article{Conlon:2010ji,
      author         = "Conlon, Joseph P. and Pedro, Francisco G.",
      title          = "{Moduli Redefinitions and Moduli Stabilisation}",
      journal        = "JHEP",
      volume         = "1006",
      pages          = "082",
      doi            = "10.1007/JHEP06(2010)082",
      year           = "2010",
      eprint         = "1003.0388",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "OUTP-10-06P",
      SLACcitation   = "%%CITATION = ARXIV:1003.0388;%%",
}



@article{Choi:2010gm,
      author         = "Choi, Kiwoon and Nilles, Hans Peter and Shin, Chang Sub
                        and Trapletti, Michele",
      title          = "{Sparticle Spectrum of Large Volume Compactification}",
      journal        = "JHEP",
      volume         = "1102",
      pages          = "047",
      doi            = "10.1007/JHEP02(2011)047",
      year           = "2011",
      eprint         = "1011.0999",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1011.0999;%%",
}



@article{Shin:2011uk,
      author         = "Shin, Chang Sub",
      title          = "{Anomalous U(1) Mediation in Large Volume
                        Compactification}",
      journal        = "JHEP",
      volume         = "1201",
      pages          = "084",
      doi            = "10.1007/JHEP01(2012)084",
      year           = "2012",
      eprint         = "1108.5740",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1108.5740;%%",
}



@article{Aldazabal:2000sa,
      author         = "Aldazabal, G. and Ibanez, Luis E. and Quevedo, F. and
                        Uranga, A.M.",
      title          = "{D-branes at singularities: A Bottom up approach to the
                        string embedding of the standard model}",
      journal        = "JHEP",
      volume         = "0008",
      pages          = "002",
      doi            = "10.1088/1126-6708/2000/08/002",
      year           = "2000",
      eprint         = "hep-th/0005067",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "FTUAM-00-10, IFT-UAM-CSIC-00-18, DAMTP-2000-42,
                        CAB-IB-2405300, CERN-TH-2000-127",
      SLACcitation   = "%%CITATION = HEP-TH/0005067;%%",
}



@article{Blumenhagen:2007sm,
      author         = "Blumenhagen, Ralph and Moster, Sebastian and Plauschinn,
                        Erik",
      title          = "{Moduli Stabilisation versus Chirality for MSSM like Type
                        IIB Orientifolds}",
      journal        = "JHEP",
      volume         = "0801",
      pages          = "058",
      doi            = "10.1088/1126-6708/2008/01/058",
      year           = "2008",
      eprint         = "0711.3389",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "MPP-2007-169",
      SLACcitation   = "%%CITATION = ARXIV:0711.3389;%%",
}



@article{Aldazabal:2000sk,
      author         = "Aldazabal, G. and Ibanez, Luis E. and Quevedo, F.",
      title          = "{A $D^-$ brane alternative to the MSSM}",
      journal        = "JHEP",
      volume         = "0002",
      pages          = "015",
      doi            = "10.1088/1126-6708/2000/02/015",
      year           = "2000",
      eprint         = "hep-ph/0001083",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FTUAM-00-001, IFT-UAM-CSIC-00-02, DAMTP-2000-01",
      SLACcitation   = "%%CITATION = HEP-PH/0001083;%%",
}



@article{Cicoli:2011qg,
      author         = "Cicoli, Michele and Mayrhofer, Christoph and Valandro,
                        Roberto",
      title          = "{Moduli Stabilisation for Chiral Global Models}",
      journal        = "JHEP",
      volume         = "1202",
      pages          = "062",
      doi            = "10.1007/JHEP02(2012)062",
      year           = "2012",
      eprint         = "1110.3333",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DESY-11-179, ZMP-HH-11-15",
      SLACcitation   = "%%CITATION = ARXIV:1110.3333;%%",
}



@article{Conlon:2007xv,
      author         = "Conlon, J.P. and Kom, C.H. and Suruliz, K. and Allanach,
                        B.C. and Quevedo, F.",
      title          = "{Sparticle Spectra and LHC Signatures for Large Volume
                        String Compactifications}",
      journal        = "JHEP",
      volume         = "0708",
      pages          = "061",
      doi            = "10.1088/1126-6708/2007/08/061",
      year           = "2007",
      eprint         = "0704.3403",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DAMTP-2007-33",
      SLACcitation   = "%%CITATION = ARXIV:0704.3403;%%",
}

@article{Schmaltz:2000gy,
      author         = "Schmaltz, Martin and Skiba, Witold",
      title          = "{Minimal gaugino mediation}",
      journal        = "Phys.Rev.",
      volume         = "D62",
      pages          = "095005",
      doi            = "10.1103/PhysRevD.62.095005",
      year           = "2000",
      eprint         = "hep-ph/0001172",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SLAC-PUB-8325, UCSD-PTH-00-01",
      SLACcitation   = "%%CITATION = HEP-PH/0001172;%%",
}

@article{Hebecker:2012qp,
      author         = "Hebecker, Arthur and Knochel, Alexander K. and Weigand,
                        Timo",
      title          = "{A Shift Symmetry in the Higgs Sector: Experimental Hints
                        and Stringy Realizations}",
      journal        = "JHEP",
      volume         = "1206",
      pages          = "093",
      doi            = "10.1007/JHEP06(2012)093",
      year           = "2012",
      eprint         = "1204.2551",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1204.2551;%%",
}

@article{Yanagida:2013ah,
      author         = "Yanagida, Tsutomu T. and Yokozaki, Norimi",
      title          = "{Focus Point in Gaugino Mediation ~ Reconsideration of
                        the Fine-tuning Problem ~}",
      journal        = "Phys.Lett.",
      volume         = "B722",
      pages          = "355-359",
      doi            = "10.1016/j.physletb.2013.04.043",
      year           = "2013",
      eprint         = "1301.1137",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1301.1137;%%",
}


@article{Conlon:2007dw,
      author         = "Conlon, Joseph P.",
      title          = "{Mirror Mediation}",
      journal        = "JHEP",
      volume         = "0803",
      pages          = "025",
      doi            = "10.1088/1126-6708/2008/03/025",
      year           = "2008",
      eprint         = "0710.0873",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2007-86",
      SLACcitation   = "%%CITATION = ARXIV:0710.0873;%%",
}
@article{Camara:2013fta,
      author         = "Camara, Pablo G. and Ibanez, Luis E. and Valenzuela,
                        Irene",
      title          = "{The String Origin of SUSY Flavor Violation}",
      journal        = "JHEP",
      volume         = "1310",
      pages          = "092",
      doi            = "10.1007/JHEP10(2013)092",
      year           = "2013",
      eprint         = "1307.3104",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "IFT-UAM-CSIC-13-081, FTUAM-13-19",
      SLACcitation   = "%%CITATION = ARXIV:1307.3104;%%",
}
@article{Baumann:2006th,
      author         = "Baumann, Daniel and Dymarsky, Anatoly and Klebanov, Igor
                        R. and Maldacena, Juan Martin and McAllister, Liam P. and
                        others",
      title          = "{On D3-brane Potentials in Compactifications with Fluxes
                        and Wrapped D-branes}",
      journal        = "JHEP",
      volume         = "0611",
      pages          = "031",
      doi            = "10.1088/1126-6708/2006/11/031",
      year           = "2006",
      eprint         = "hep-th/0607050",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "PUPT-2202, ITEP-TH-32-06",
      SLACcitation   = "%%CITATION = HEP-TH/0607050;%%",
}
@article{Gukov:1999ya,
      author         = "Gukov, Sergei and Vafa, Cumrun and Witten, Edward",
      title          = "{CFT's from Calabi-Yau four folds}",
      journal        = "Nucl.Phys.",
      volume         = "B584",
      pages          = "69-108",
      doi            = "10.1016/S0550-3213(00)00373-4",
      year           = "2000",
      eprint         = "hep-th/9906070",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "HUTP-99-A034, IASSNS-HEP-99-52, PUPT-1864",
      SLACcitation   = "%%CITATION = HEP-TH/9906070;%%",
}

@article{Burgess:2010bz,
      author         = "Burgess, C.P. and Cicoli, M. and Gomez-Reino, M. and
                        Quevedo, F. and Tasinato, G. and others",
      title          = "{Non-standard primordial fluctuations and nongaussianity
                        in string inflation}",
      journal        = "JHEP",
      volume         = "1008",
      pages          = "045",
      doi            = "10.1007/JHEP08(2010)045",
      year           = "2010",
      eprint         = "1005.4840",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2010-44, DESY-10-071",
      SLACcitation   = "%%CITATION = ARXIV:1005.4840;%%",
}

@article{Cicoli:2012vw,
      author         = "Cicoli, Michele and Krippendorf, Sven and Mayrhofer,
                        Christoph and Quevedo, Fernando and Valandro, Roberto",
      title          = "{D-Branes at del Pezzo Singularities: Global Embedding
                        and Moduli Stabilisation}",
      journal        = "JHEP",
      volume         = "1209",
      pages          = "019",
      doi            = "10.1007/JHEP09(2012)019",
      year           = "2012",
      eprint         = "1206.5237",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2012-47, ZMP-HH-12-10",
      SLACcitation   = "%%CITATION = ARXIV:1206.5237;%%",
}

@article{Cicoli:2012fh,
      author         = "Cicoli, Michele and Maharana, Anshuman and Quevedo, F.
                        and Burgess, C.P.",
      title          = "{De Sitter String Vacua from Dilaton-dependent
                        Non-perturbative Effects}",
      journal        = "JHEP",
      volume         = "1206",
      pages          = "011",
      doi            = "10.1007/JHEP06(2012)011",
      year           = "2012",
      eprint         = "1203.1750",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2012-7",
      SLACcitation   = "%%CITATION = ARXIV:1203.1750;%%",
}



@article{Grana:2002nq,
      author         = "Grana, Mariana",
      title          = "{MSSM parameters from supergravity backgrounds}",
      journal        = "Phys.Rev.",
      volume         = "D67",
      pages          = "066006",
      doi            = "10.1103/PhysRevD.67.066006",
      year           = "2003",
      eprint         = "hep-th/0209200",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = HEP-TH/0209200;%%",
}

@article{Berenstein:2005xa,
      author         = "Berenstein, D. and Herzog, C.P. and Ouyang, P. and
                        Pinansky, S.",
      title          = "{Supersymmetry breaking from a Calabi-Yau singularity}",
      journal        = "JHEP",
      volume         = "0509",
      pages          = "084",
      doi            = "10.1088/1126-6708/2005/09/084",
      year           = "2005",
      eprint         = "hep-th/0505029",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "NSF-KITP-05-27",
      SLACcitation   = "%%CITATION = HEP-TH/0505029;%%",
}



@article{Grana:2003ek,
      author         = "Grana, Mariana and Grimm, Thomas W. and Jockers, Hans and
                        Louis, Jan",
      title          = "{Soft supersymmetry breaking in Calabi-Yau orientifolds
                        with D-branes and fluxes}",
      journal        = "Nucl.Phys.",
      volume         = "B690",
      pages          = "21-61",
      doi            = "10.1016/j.nuclphysb.2004.04.021",
      year           = "2004",
      eprint         = "hep-th/0312232",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "CPHT-RR-116-1203",
      SLACcitation   = "%%CITATION = HEP-TH/0312232;%%",
}

@article{Dudas:2005vv,
      author         = "Dudas, Emilian and Vempati, Sudhir K.",
      title          = "{Large D-terms, hierarchical soft spectra and moduli
                        stabilisation}",
      journal        = "Nucl.Phys.",
      volume         = "B727",
      pages          = "139-162",
      doi            = "10.1016/j.nuclphysb.2005.08.034",
      year           = "2005",
      eprint         = "hep-th/0506172",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "CPHT-RR-024-0405, LPT-ORSAY-05-27",
      SLACcitation   = "%%CITATION = HEP-TH/0506172;%%",
}

@article{Cicoli:2013cha,
      author         = "Cicoli, Michele and Klevers, Denis and Krippendorf, Sven
                        and Mayrhofer, Christoph and Quevedo, Fernando and others",
      title          = "{Explicit de Sitter Flux Vacua for Global String Models
                        with Chiral Matter}",
      journal        = "JHEP",
      volume         = "1405",
      pages          = "001",
      doi            = "10.1007/JHEP05(2014)001",
      year           = "2014",
      eprint         = "1312.0014",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1312.0014;%%",
}
@article{Antoniadis:1994hg,
      author         = "Antoniadis, Ignatios and Gava, E. and Narain, K.S. and
                        Taylor, T.R.",
      title          = "{Effective mu term in superstring theory}",
      journal        = "Nucl.Phys.",
      volume         = "B432",
      pages          = "187-204",
      doi            = "10.1016/0550-3213(94)90599-1",
      year           = "1994",
      eprint         = "hep-th/9405024",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "NUB-3084, IC-94-72, CPTH-A282-0194",
      SLACcitation   = "%%CITATION = HEP-TH/9405024;%%",
}
@article{LopesCardoso:1994is,
      author         = "Lopes Cardoso, Gabriel and Lust, Dieter and Mohaupt,
                        Thomas",
      title          = "{Moduli spaces and target space duality symmetries in
                        (0,2) Z(N) orbifold theories with continuous Wilson
                        lines}",
      journal        = "Nucl.Phys.",
      volume         = "B432",
      pages          = "68-108",
      doi            = "10.1016/0550-3213(94)90594-0",
      year           = "1994",
      eprint         = "hep-th/9405002",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "HUB-IEP-94-6, DESY-94-080",
      SLACcitation   = "%%CITATION = HEP-TH/9405002;%%",
}
@article{LoaizaBrito:2005fa,
      author         = "Loaiza-Brito, Oscar and Martin, Johannes and Nilles, Hans
                        Peter and Ratz, Michael",
      title          = "{Log(M(Pl) / m(3/2))}",
      journal        = "AIP Conf.Proc.",
      volume         = "805",
      pages          = "198-204",
      doi            = "10.1063/1.2149698",
      year           = "2006",
      eprint         = "hep-th/0509158",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = HEP-TH/0509158;%%",
}
@article{Brignole:1995fb,
      author         = "Brignole, A. and Ibanez, Luis E. and Munoz, C. and
                        Scheich, C.",
      title          = "{Some issues in soft SUSY breaking terms from dilaton /
                        moduli sectors}",
      journal        = "Z.Phys.",
      volume         = "C74",
      pages          = "157-170",
      doi            = "10.1007/s002880050379",
      year           = "1997",
      eprint         = "hep-ph/9508258",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FTUAM-95-26, LBL-37564",
      SLACcitation   = "%%CITATION = HEP-PH/9508258;%%",
}
@article{Brignole:1996xb,
      author         = "Brignole, A. and Ibanez, Luis E. and Munoz, C.",
      title          = "{Orbifold induced mu term and electroweak symmetry
                        breaking}",
      journal        = "Phys.Lett.",
      volume         = "B387",
      pages          = "769-774",
      doi            = "10.1016/0370-2693(96)01114-8",
      year           = "1996",
      eprint         = "hep-ph/9607405",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-TH-96-183, FTUAM-96-28",
      SLACcitation   = "%%CITATION = HEP-PH/9607405;%%",
}
@article{Kim:1983dt,
      author         = "Kim, Jihn E. and Nilles, Hans Peter",
      title          = "{The mu Problem and the Strong CP Problem}",
      journal        = "Phys.Lett.",
      volume         = "B138",
      pages          = "150",
      doi            = "10.1016/0370-2693(84)91890-2",
      year           = "1984",
      reportNumber   = "UGVA-DPT 1983/10-410",
      SLACcitation   = "%%CITATION = PHLTA,B138,150;%%",
}
@article{Giudice:1988yz,
      author         = "Giudice, G.F. and Masiero, A.",
      title          = "{A Natural Solution to the mu Problem in Supergravity
                        Theories}",
      journal        = "Phys.Lett.",
      volume         = "B206",
      pages          = "480-484",
      doi            = "10.1016/0370-2693(88)91613-9",
      year           = "1988",
      reportNumber   = "SISSA-17/88/EP",
      SLACcitation   = "%%CITATION = PHLTA,B206,480;%%",
}
@article{Cicoli:2013mpa,
      author         = "Cicoli, Michele and Krippendorf, Sven and Mayrhofer,
                        Christoph and Quevedo, Fernando and Valandro, Roberto",
      title          = "{D3/D7 Branes at Singularities: Constraints from Global
                        Embedding and Moduli Stabilisation}",
      journal        = "JHEP",
      volume         = "1307",
      pages          = "150",
      doi            = "10.1007/JHEP07(2013)150",
      year           = "2013",
      eprint         = "1304.0022",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1304.0022;%%",
}



@article{Krippendorf:2009zza,
      author         = "Krippendorf, Sven and Quevedo, Fernando",
      title          = "{Metastable SUSY Breaking, de Sitter Moduli Stabilisation
                        and Kahler Moduli Inflation}",
      journal        = "JHEP",
      volume         = "0911",
      pages          = "039",
      doi            = "10.1088/1126-6708/2009/11/039",
      year           = "2009",
      eprint         = "0901.0683",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:0901.0683;%%",
}



@article{Cicoli:2008va,
      author         = "Cicoli, Michele and Conlon, Joseph P. and Quevedo,
                        Fernando",
      title          = "{General Analysis of LARGE Volume Scenarios with String
                        Loop Moduli Stabilisation}",
      journal        = "JHEP",
      volume         = "0810",
      pages          = "105",
      doi            = "10.1088/1126-6708/2008/10/105",
      year           = "2008",
      eprint         = "0805.1029",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2008-16",
      SLACcitation   = "%%CITATION = ARXIV:0805.1029;%%",
}



@article{Kaplunovsky:1993rd,
      author         = "Kaplunovsky, Vadim S. and Louis, Jan",
      title          = "{Model independent analysis of soft terms in effective
                        supergravity and in string theory}",
      journal        = "Phys.Lett.",
      volume         = "B306",
      pages          = "269-275",
      doi            = "10.1016/0370-2693(93)90078-V",
      year           = "1993",
      eprint         = "hep-th/9303040",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "CERN-TH-6809-93, UTTG-05-93",
      SLACcitation   = "%%CITATION = HEP-TH/9303040;%%",
}
@article{Kaplan:1999ac,
      author         = "Kaplan, D. Elazzar and Kribs, Graham D. and Schmaltz,
                        Martin",
      title          = "{Supersymmetry breaking through transparent extra
                        dimensions}",
      journal        = "Phys.Rev.",
      volume         = "D62",
      pages          = "035010",
      doi            = "10.1103/PhysRevD.62.035010",
      year           = "2000",
      eprint         = "hep-ph/9911293",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SLAC-PUB-8291, FERMILAB-PUB-99-327-T, ANL-HEP-PR-99-110,
                        EFI-99-48",
      SLACcitation   = "%%CITATION = HEP-PH/9911293;%%",
}

@article{Coughlan:1983ci,
      author         = "Coughlan, G.D. and Fischler, W. and Kolb, Edward W. and
                        Raby, S. and Ross, Graham G.",
      title          = "{Cosmological Problems for the Polonyi Potential}",
      journal        = "Phys.Lett.",
      volume         = "B131",
      pages          = "59",
      doi            = "10.1016/0370-2693(83)91091-2",
      year           = "1983",
      reportNumber   = "LA-UR-83-1423",
      SLACcitation   = "%%CITATION = PHLTA,B131,59;%%",
}

@article{Banks:1993en,
      author         = "Banks, Tom and Kaplan, David B. and Nelson, Ann E.",
      title          = "{Cosmological implications of dynamical supersymmetry
                        breaking}",
      journal        = "Phys.Rev.",
      volume         = "D49",
      pages          = "779-787",
      doi            = "10.1103/PhysRevD.49.779",
      year           = "1994",
      eprint         = "hep-ph/9308292",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCSD-PTH-93-26, RU-37",
      SLACcitation   = "%%CITATION = HEP-PH/9308292;%%",
}


@article{deCarlos:1993jw,
      author         = "de Carlos, B. and Casas, J.A. and Quevedo, F. and Roulet,
                        E.",
      title          = "{Model independent properties and cosmological
                        implications of the dilaton and moduli sectors of 4-d
                        strings}",
      journal        = "Phys.Lett.",
      volume         = "B318",
      pages          = "447-456",
      doi            = "10.1016/0370-2693(93)91538-X",
      year           = "1993",
      eprint         = "hep-ph/9308325",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-TH-6958-93, NEIP-93-006, IEM-FT-75-93",
      SLACcitation   = "%%CITATION = HEP-PH/9308325;%%",
}

@article{Cicoli:2011yh,
      author         = "Cicoli, Michele and Goodsell, Mark and Jaeckel, Joerg and
                        Ringwald, Andreas",
      title          = "{Testing String Vacua in the Lab: From a Hidden CMB to
                        Dark Forces in Flux Compactifications}",
      journal        = "JHEP",
      volume         = "1107",
      pages          = "114",
      doi            = "10.1007/JHEP07(2011)114",
      year           = "2011",
      eprint         = "1103.3705",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DESY-11-042, IPPP-11-13, DCTP-11-26",
      SLACcitation   = "%%CITATION = ARXIV:1103.3705;%%",
}

@article{Chacko:1999mi,
      author         = "Chacko, Z. and Luty, Markus A. and Nelson, Ann E. and
                        Ponton, Eduardo",
      title          = "{Gaugino mediated supersymmetry breaking}",
      journal        = "JHEP",
      volume         = "0001",
      pages          = "003",
      doi            = "10.1088/1126-6708/2000/01/003",
      year           = "2000",
      eprint         = "hep-ph/9911323",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UMD-PP-00-040, UW-PT-99-26",
      SLACcitation   = "%%CITATION = HEP-PH/9911323;%%",
}

@article{Brignole:1993dj,
      author         = "Brignole, A. and Ibanez, Luis E. and Munoz, C.",
      title          = "{Towards a theory of soft terms for the supersymmetric
                        Standard Model}",
      journal        = "Nucl.Phys.",
      volume         = "B422",
      pages          = "125-171",
      doi            = "10.1016/0550-3213(94)00068-9",
      year           = "1994",
      eprint         = "hep-ph/9308271",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FTUAM-26-93",
      SLACcitation   = "%%CITATION = HEP-PH/9308271;%%",
}



@article{Ellis:1986nr,
      author         = "Ellis, John R. and Lahanas, A.B. and Nanopoulos, Dimitri
                        V. and Quiros, M. and Zwirner, F.",
      title          = "{Supersymmetry Breaking in the Observable Sector of
                        Superstring Models}",
      journal        = "Phys.Lett.",
      volume         = "B188",
      pages          = "408",
      doi            = "10.1016/0370-2693(87)91639-X",
      year           = "1987",
      reportNumber   = "CERN-TH-4626/86, MAD/TH/86-33",
      SLACcitation   = "%%CITATION = PHLTA,B188,408;%%",
}



@article{Antoniadis:1997ic,
      author         = "Antoniadis, Ignatios and Quiros, M.",
      title          = "{Supersymmetry breaking in M theory and gaugino
                        condensation}",
      journal        = "Nucl.Phys.",
      volume         = "B505",
      pages          = "109-122",
      doi            = "10.1016/S0550-3213(97)00490-2",
      year           = "1997",
      eprint         = "hep-th/9705037",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "CERN-TH-97-090, CERN-TH-97-90, CPTH-S504-0497,
                        IEM-FT-154-97",
      SLACcitation   = "%%CITATION = HEP-TH/9705037;%%",
}



@article{Lee:2013aia,
      author         = "Lee, Jae Yong",
      title          = "{Gaugino masses from gravitino at one loop}",
      year           = "2013",
      eprint         = "1302.5846",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1302.5846;%%",
}



@article{Bagger:1999rd,
      author         = "Bagger, Jonathan A. and Moroi, Takeo and Poppitz, Erich",
      title          = "{Anomaly mediation in supergravity theories}",
      journal        = "JHEP",
      volume         = "0004",
      pages          = "009",
      doi            = "10.1088/1126-6708/2000/04/009",
      year           = "2000",
      eprint         = "hep-th/9911029",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "IASSNS-HEP-99-89, YCTP-P27-99",
      SLACcitation   = "%%CITATION = HEP-TH/9911029;%%",
}



@article{deAlwis:2008aq,
      author         = "de Alwis, S.P.",
      title          = "{On Anomaly Mediated SUSY Breaking}",
      journal        = "Phys.Rev.",
      volume         = "D77",
      pages          = "105020",
      doi            = "10.1103/PhysRevD.77.105020",
      year           = "2008",
      eprint         = "0801.0578",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "COLO-HEP-528",
      SLACcitation   = "%%CITATION = ARXIV:0801.0578;%%",
}



@article{Conlon:2010qy,
      author         = "Conlon, Joseph P. and Goodsell, Mark and Palti, Eran",
      title          = "{Anomaly Mediation in Superstring Theory}",
      journal        = "Fortsch.Phys.",
      volume         = "59",
      pages          = "5-75",
      doi            = "10.1002/prop.201000087",
      year           = "2011",
      eprint         = "1008.4361",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "CPHT-RR056.0810, DESY-10-135, OUTP-10-21P",
      SLACcitation   = "%%CITATION = ARXIV:1008.4361;%%",
}



@article{1106.6039,
      author         = "Dolan, Matthew J. and Krippendorf, Sven and Quevedo,
                        Fernando",
      title          = "{Towards a Systematic Construction of Realistic D-brane
                        Models on a del Pezzo Singularity}",
      journal        = "JHEP",
      volume         = "1110",
      pages          = "024",
      doi            = "10.1007/JHEP10(2011)024",
      year           = "2011",
      eprint         = "1106.6039",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1106.6039;%%",
}



@article{1002.1790,
      author         = "Krippendorf, Sven and Dolan, Matthew J. and Maharana,
                        Anshuman and Quevedo, Fernando",
      title          = "{D-branes at Toric Singularities: Model Building, Yukawa
                        Couplings and Flavour Physics}",
      journal        = "JHEP",
      volume         = "1006",
      pages          = "092",
      doi            = "10.1007/JHEP06(2010)092",
      year           = "2010",
      eprint         = "1002.1790",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1002.1790;%%",
}



@article{1111.3047,
      author         = "Maharana, Anshuman",
      title          = "{Symmetry Breaking Bulk Effects in Local D-brane Models}",
      journal        = "JHEP",
      volume         = "1206",
      pages          = "002",
      doi            = "10.1007/s13130-012-4129-0, 10.1007/JHEP06(2012)002",
      year           = "2012",
      eprint         = "1111.3047",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2011-101",
      SLACcitation   = "%%CITATION = ARXIV:1111.3047;%%",
}



@article{0810.5660,
      author         = "Conlon, Joseph P. and Maharana, Anshuman and Quevedo,
                        Fernando",
      title          = "{Towards Realistic String Vacua}",
      journal        = "JHEP",
      volume         = "0905",
      pages          = "109",
      doi            = "10.1088/1126-6708/2009/05/109",
      year           = "2009",
      eprint         = "0810.5660",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "OUTP-08-18P, DAMTP-2008-101, CERN-PH-TH-2008-214",
      SLACcitation   = "%%CITATION = ARXIV:0810.5660;%%",
}

@article{Ade:2014xna,
      author         = "Ade, P.A.R. and others",
      title          = "{BICEP2 I: Detection Of B-mode Polarization at Degree
                        Angular Scales}",
      collaboration  = "BICEP2 Collaboration",
      year           = "2014",
      eprint         = "1403.3985",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1403.3985;%%",
}

@article{Junghans:2014zla,
      author         = "Junghans, Daniel and Shiu, Gary",
      title          = "{Brane Curvature Corrections to the $\mathcal{N}=1$ Type
                        II/F-theory Effective Action}",
      year           = "2014",
      eprint         = "1407.0019",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "MAD-TH-13-07",
      SLACcitation   = "%%CITATION = ARXIV:1407.0019;%%",
}


@article{us,
author = " Aparicio, Luis and Cicoli, Michele and Krippendorf, Sven and Maharana, Anshuman and Muia, Francesco and Quevedo, Fernando",
title = "   {Sequestered de Sitter String Models:  LHC Phenomenology}",
journal = "to appear",
}

@article{Ibanez:2013gf,
      author         = "Ibanez, Luis E. and Valenzuela, Irene",
      title          = "{The Higgs Mass as a Signature of Heavy SUSY}",
      journal        = "JHEP",
      volume         = "1305",
      pages          = "064",
      doi            = "10.1007/JHEP05(2013)064",
      year           = "2013",
      eprint         = "1301.5167",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-UAM-CSIC-13-008, FTUAM-13-126",
      SLACcitation   = "%%CITATION = ARXIV:1301.5167;%%",
}

@article{Conlon:2006us,
      author         = "Conlon, Joseph P. and Quevedo, Fernando",
      title          = "{Gaugino and Scalar Masses in the Landscape}",
      journal        = "JHEP",
      volume         = "0606",
      pages          = "029",
      doi            = "10.1088/1126-6708/2006/06/029",
      year           = "2006",
      eprint         = "hep-th/0605141",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2006-37",
      SLACcitation   = "%%CITATION = HEP-TH/0605141;%%",
}

@article{Conlon:2006wz,
      author         = "Conlon, Joseph P. and Abdussalam, Shehu S. and Quevedo,
                        Fernando and Suruliz, Kerim",
      title          = "{Soft SUSY Breaking Terms for Chiral Matter in IIB String
                        Compactifications}",
      journal        = "JHEP",
      volume         = "0701",
      pages          = "032",
      doi            = "10.1088/1126-6708/2007/01/032",
      year           = "2007",
      eprint         = "hep-th/0610129",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2006-89",
      SLACcitation   = "%%CITATION = HEP-TH/0610129;%%",
}

@article{deAlwis:2009fn,
      author         = "de Alwis, S.P.",
      title          = "{Classical and Quantum SUSY Breaking Effects in IIB Local
                        Models}",
      journal        = "JHEP",
      volume         = "1003",
      pages          = "078",
      doi            = "10.1007/JHEP03(2010)078",
      year           = "2010",
      eprint         = "0912.2950",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "COLO-HEP-549",
      SLACcitation   = "%%CITATION = ARXIV:0912.2950;%%",
}

